Distributed Learning in Ad-Hoc Networks: A Multi-player Multi-armed Bandit Framework

Next-generation networks are expected to be ultra-dense with a very high peak rate but relatively lower expected traffic per user. For such scenario, existing central controller based resource allocation may incur substantial signaling (control communications) leading to a negative effect on the quality of service (e.g. drop calls), energy and spectrum efficiency. To overcome this problem, cognitive ad-hoc networks (CAHN) that share spectrum with other networks are being envisioned. They allow some users to identify and communicate in `free slots' thereby reducing signaling load and allowing the higher number of users per base stations (dense networks). Such networks open up many interesting challenges such as resource identification, coordination, dynamic and context-aware adaptation for which Machine Learning and Artificial Intelligence framework offers novel solutions. In this paper, we discuss state-of-the-art multi-armed multi-player bandit based distributed learning algorithms that allow users to adapt to the environment and coordinate with other players/users. We also discuss various open research problems for feasible realization of CAHN and interesting applications in other domains such as energy harvesting, Internet of Things, and Smart grids.

==> asymmetric_network.tex <==
Heterogeneous channels channels \\

==> malicious_users.tex <==
jammers \\

==> network_model.tex <==

	Consider a network consisting of $U$ number of SUs without any central
control and communication among them and $N$ channels such that $N > U$ . We assume time slotted communication where the horizon is divided into $T$ number of time slots, i.e., $t \in \{1,2,..,T\}$. The reward of the channel $i\in[N]$ is sampled independently from some distribution on [0,1] with expected reward $\mu_i$. In every time slot, a SU selects a channel  and would like to receive the highest cumulative reward in $T$ time slots overall. Same set-up has been considered for non-cooperative cognitive radio network network in many works including \cite{MC,MEGA}. \par
In our model, 
we assume that a SU does not
possess knowledge of the total number of active SUs in the network. We
denote the top $K$ channels as the set of $K$ channels with the
highest expected rewards. For simplicity of analysis, we assume
ideal detector, i.e. no sensing error. When more than one SU select the same vacant channel, collision occurs. If no collusion occurs, data transmission is considered to be successful.\par


	 We evaluate the performance of our algorithms in terms of expected regret defined as the difference of expected optimal throughput and runtime average throughput defined as follows: 
	 
	 \begin{align} \label{eq:regret} 
	 Regret &= R_{op}-\sum\limits_{t=1}^{T}\sum\limits_{u=1}^{U} \mu_{I_t^u}(1- E\left[C_{I_t^u}^u\right]).	 
	 \end{align}
	where $R_{op}$ is the maximum mean total throughput achievable for SUs. It is achieved when each SU transmits on one of the top channels and do not collide with each other. $I_t^u$ denotes the channel selected by SU $u$ at time $t$. $\mu_{I_t^u}$  and $C_{I_t^u}^u$ denote the expected reward and collision indicator on channel  $I_t^u$, respectively. If there is collision, collision indicator is set to $1$, otherwise it is $0$. 
	 
The average number of collisions, $C_T$, is given by
\begin{equation}
\label{coll}
C_T=\sum_{t=1}^T\sum_{u=1}^U \mathbb{E}[C_{I_t^u}^u].
\end{equation}

		Our goal is to design distributed algorithm that keeps regret and $C_T$ as small as possible.% for static as well as dynamic networks.
%		 The various notations and their definitions are summarized in Table I.
			
	
	
%\begin{table}[!h]
%	%\centering
%	\captionsetup{justification=raggedright,singlelinecheck=false}
%	\caption{Notations and Definitions}
%	\label{gc}
%	
%	\begin{tabular}{|l|l|}
%		\hline
%		\textbf{Notations} & \textbf{Definitions} \\
%		\hline
%		$U$ & No. of SUs \\
%		\hline
%		$N$ & No. of channels\\
%		\hline
%		$t$ & Current time slot\\
%		\hline
%		$T$ & Total time horizon\\
%		\hline
%		$\mu_i^u$ & Channel vacancy probability of channel $i$ observed by  \\ & the $u^{th}$ SU \\
%		\hline
%		$\Delta$ & Gap between $n^{th}$ and $(n+1)^{th}$ channel statistics \\
%		\hline
%		$R_{op}$ & Maximum total throughput achievable            		for SUs \\
%		\hline
%		$r_t^u$ & Reward received by the $u^{th}$ SU at time $t$\\
%		
%		\hline		
%	 $I_t^u$ & Channel selected by SU $u$ at time $t$ \\
%	 \hline	
%	  $\mu_{I_t^u}$  & Vacancy probability on channel  $I_t^u$\\
%	   \hline	
%	   $C_{I_t^u}^u$ & Collision indicator on channel  $I_t^u$ \\ 
%	   \hline
%	   $C_T$ & Average number of collisions \\		
%		\hline		
%		$T_{RH}$ & Duration of the random hopping\\
%		\hline		
%		$T_{SH}$ & Duration of the sequential hopping\\
%		\hline		
%		$T_{CC}$ & Duration of the CC phase\\
%				\hline			
%		$S_n^u$ & Number of times channel $n$ is chosen by the $u^{th}$ SU \\
%		\hline
%		$V_n^u$  & Number of times channel $n$, when chosen by the \\ & $u^{th}$ SU, is found vacant\\
%		\hline
%		$C_n^u$ &  Expected number of collisions seen by the $u^{th}$ SU over \\& channel $n$ \\
%		\hline
%		$\pi^u$ & Array of the channel indices sorted in the decreasing\\ &  order of estimated channel vacancy probabilities\\
%		\hline
%		$N_i $ & Number of times channel $i$ needs to
%be sensed \\ & to guarantee that it is not occupied by another SU\\
%\hline
%$M_i $ & Number of time slots after which a SU in channel $i$ at \\ & the end of CC phase settles in next best channel\\
%\hline
%$Y_n$  &  Number of times channel $n$ is chosen by a SU \\ 
%\hline
%$\chi_n$ & Indicator to show the presence of a SU or collision in \\ & the channel $n$\\
%\hline
%$\aleph$ & Indicator to show the locking of a SU\\
%\hline
%$T_{TR}$ & Total orthogonalization time of the trekking
%approach\\
%\hline
%$T_{EN}^u$ & Time slot in which the $u^{th}$ SU enters into the network\\
%\hline
%$T_{CI}$ & Maximum number of time slots needed to enter into the \\ & TL state from OST
%state\\
%\hline
%$T_{TL}$ & Duration of TL state \\
%\hline
%$T_{OT}$ & Duration of OST state \\
%\hline
%$N_m$ & Number of SUs who enter in the network at the start \\ & of the horizon\\
%\hline
%$N_e$ & Number of SUs who enter late in the network\\
%\hline
%$N_l$ & Number of SUs leaving the network\\
%
%%		\hline
%%		$P_{f}$ & Probability for any SU to become fixed on any frequency  \\ & band \\
%%		\hline
%%		$T_{f}$ & Total time taken by any SU to become fixed on any  \\ & channel \\
%%		\hline
%%		$C_{u}$ & Number of SU collisions faced by $u^{th}$ SU \\
%		\hline
%		
%	\end{tabular}
%\end{table}	

==> prevwork.tex <==

Finding a solution for the multi-user CRN-MAB problem has received significant attention in last few years. The  $\rho^{rand}$ \cite{prand} algorithm employs upper confidence bound (UCB) based multi-armed bandit (MAB) algorithm to identify optimal channels and random rank selection for SU orthogonalization. The distributed learning algorithm with Fairness (DLF) algorithm in \cite{gai2} shows to offer improved regret than \cite{prand} using advanced MAB algorithm. Using larger subset of channels than top $U$ channels during exploration, \cite{zandi} reduces the number of collisions.  In \cite{zhandi}, $\rho^{rand}$ algorithm is improved by replacing randomization approach for rank selection with the learning based approach. Though the algorithm in \cite{prand,gai2,zhandi,zandi} provide a coordination and communication free algorithms for multi-user CRN-MAB problem but they rely on exact knowledge of the number of SUs in the network. However, in modelling problems such as cognitive radio networks these are not always realistic assumptions. In addition, they offer lower regret and fewer number of SU collisions making it non-suitable suitable for battery operated SUs in the CRN. The algorithm In \cite{quek} based on two-stage channel access scheme with common hopping sequence guarantees negligible number of SU collisions but it has the drawback that the SUs select all channels uniformly leading to high regret. \par 


The works most similar to ours in spirit are multiuser $\epsilon$ - greedy collision avoiding  (MEGA) \cite{MEGA} and musical chair (MC) \cite{MC} which do not need prior knowledge of $U$. It has been shown in \cite{MC} that the MC algorithm outperforms MEGA algorithm and is computationally efficient. The drawbacks of MC algorithm are that it incurs significant number of collisions before it learns the number of users in the networks as well as  random selection approach in the learning stage makes the rendezvous, i.e. the process of SU transmitter and receiver tuning themselves to communicate on an identical channel, challenging. The proposed algorithm presented in next section aims to overcome these shortcomings.

	 

==> simulation_results.tex <==
We present the simulation results to compare the performance of the proposed algorithm with Distributed Learning Algorithm with Fairness (DLF) \cite{gai2}, its variant with unknown $U$ (DLF-Un), MC algorithm \cite{MC} and algorithm in \cite{quek}. We consider $N=8$ and $\mu_n =  \{0.29,0.36,0.43,0.50,0.57,0.64,0.71,0.78\}$ with the channel statistics of $\mu_{\lceil \frac{N}{2}\rceil} = 0.5$ and the minimum gap between the statistics of the $n^{th}$ and $(n+1)^{th}$ channel, i.e. $\Delta$, is 0.07. All the numerical results are averaged over 50 independent experiments with the horizon of 10000 time slots. The values of $T_{CC}$ in the proposed algorithm and $T_O$ in the MC is 2000. \par

The vacant spectrum utilization, $S_T$ in \% for $N$ = 8 and $U =\{4,8\}$ is shown in  Fig. \ref{rd13} and \ref{rd14}. From Fig. \ref{rd13}, it is evident that the proposed algorithm utilized the vacant spectrum more efficiently than DLF-Un, MC and \cite{quek} algorithms where $U$ is unknown. Also, the performance of the proposed algorithm and algorithm in \cite{quek} improve with the increase in $U$ due to fewer number of collisions. This is interesting considering the fact that next generation networks will more likely to be dense. Due to uniform and collision-free channel selection approach, the performance of algorithm in \cite{quek} is identical to proposed algorithm for $U=N$. Note that in Fig.~\ref{rd14}, the plots for DLF and DLF-Un overlap as both are identical since $U = N$. As discussed in Section~\ref{model}, regret (i.e. loss of throughput) is another metric to compare the performance of the distributed algorithm. Fig.~\ref{rd16} and Fig.~\ref{rd17} compare the regret of various algorithms for $N=8$ and $U=\{4,8\}$, respectively. It is evident that the proposed algorithm significantly outperforms other algorithms. The constant regret after the OR phase
confirms the orthogonalization of users in the top channels which is the objective of a distributive algorithm. 

%Next, we compare the effect of $U$ on the performance of the proposed algorithm in Fig. \ref{rd31}. As expected, with increase in $U$, the difference between the regret increases. This validates analytical results presented in Section III.
The average number of collisions and hence, the number of retransmissions experienced by all users are compared in Fig.~\ref{rd3}. The $y$-axis is shown using the logarithmic scale for clarity of plots. It can be observed that the number of collisions are significantly lower in the proposed algorithm with probability of collision of 0.001. Though algorithm in \cite{quek} offers almost zero collisions, it assumes either the presence of central controller or sensing hardware. Furthermore, the regret of \cite{quek} is significantly poor than the proposed algorithm. 

%Next, we compare the average number of collisions, $C_T$, faced by all users  at the end of the horizon i.e. after 10000 transmission attempts by each user. As shown in Fig.~\ref{rd3} with the data on $y-axis$ represented using logarithmic scale, the number of collisions are negligible in the proposed algorithm. In case of \cite{quek}, the number of user collisions are almost zero due to use of central controller or sensing hardware compared to at most 100 collisions in the proposed algorithm which does not need central controller or sensing hardware. Still, the probability of collision in the proposed algorithm is very small (0.001). 

Next, we compare the channel allocations among users in a single experiment. As shown in Fig.~\ref{fair}, proposed algorithm guarantees fairness in the channel allocation while in MC and DLF algorithms some users get higher priority over top channel than others. Fairness in channel allocation also guarantee same average throughput at each user. 







==> symmetric_network.tex <==
Homogeneous channels \\
